Hidden Conformal Symmetry of the Kerr Black Hole

Extreme and very-near-extreme spin J Kerr black holes have been conjectured to be holographically dual to two-dimensional (2D) conformal field theories (CFTs) with left and right central charges c_L=c_R=12J. In this paper it is observed that the 2D conformal symmetry of the scalar wave equation at low frequencies persists for generic non-extreme values of the mass M. Interestingly, this conformal symmetry is not derived from a conformal symmetry of the spacetime geometry except in the extreme limit. The periodic identification of the azimuthal angle is shown to correspond to a spontaneous breaking of the conformal symmetry by left and right temperatures (T_L,T_R). The well-known low-frequency scalar-Kerr scattering amplitudes coincide with correlators of a 2D CFT at these temperatures. Moreover the CFT microstate degeneracy inferred from the Cardy formula agrees exactly with the Bekenstein-Hawking area law for all M and J. These observations provide evidence for the conjecture that the Kerr black hole is dual to a c_L=c_R=12J 2D CFT at temperatures (T_L,T_R) for every value of M and J.

==> toc.tex <==
\noindent {1.} {Introduction} \leaderfill{1} \par 
\noindent {2.} {Massless Scalar Wave Equation} \leaderfill{3} \par 
\noindent {3.} {The Near Region } \leaderfill{5} \par 
\noindent {4.} {$SL(2,R)_L\times SL(2,R)_R$} \leaderfill{6} \par 
\noindent {5.} {CFT Interpretation} \leaderfill{8} \par 
\noindent \quad{5.1.} {Temperature} \leaderfill{8} \par 
\noindent \quad{5.2.} {Entropy} \leaderfill{9} \par 
\noindent {6.} {Scattering} \leaderfill{10} \par 
\noindent \quad{6.1.} {Absorption Probabilities} \leaderfill{10} \par 
\noindent \quad{6.2.} {Parameter Ranges} \leaderfill{12} \par 

